Efficient Algorithms for Interdicting Facilities in Trees and Bounded Treewidth Graphs

Given a graph $G$ of $n$ nodes partitioned into facilities and customers, the $r$-edge interdiction covering problem (REIC) is to remove up to $r$ edges so as to maximize the total weight of customers disconnected from all facilities, which is called the covering objective function. While REIC is known to be NP-complete for general graphs, Fr\"ohlich and Ruzika show that the problem can be solved in polynomial time when $G$ is a tree, providing an $O(n^7 r)$-time algorithm. We give an efficient $O(nr^2)$-time dynamic programming algorithm for REIC on trees that is fixed-parameter linear in $n$. Evaluating our solution on a benchmark of randomly generated tree networks with baselines of the Fr\"ohlich and Ruzika algorithm and the Gurobi integer program solver, we demonstrate that in practice, our algorithm is both significantly faster and less sensitive to network topology and size. We extend our algorithm for REIC to graphs of bounded treewidth, a well-studied family of sparse graphs that generalizes trees, and obtain a matching runtime of $O(nr^2)$. We also consider the $r$-facility interdiction covering problem (RFIC), a novel variant of this network interdiction problem where the goal is to remove up to $r$ facilities to maximize the covering objective function over disconnected customers. We show that RFIC is NP-complete by observing it generalizes the small set bipartite vertex expansion problem (SSBVE), also known as the minimum $p$-union problem. We give an $O(nr^2)$-time algorithm for RFIC on trees, which also gives an $O(n^3)$-time algorithm for SSBVE on trees.

==> sections/6_courcelles.tex <==
\section{Discussion of Courcelle's Theorem}
\label{sec:courcelle}
In this section, we make a theoretical and practical comparison of our fixed-parameter linear DP algorithms for REIC to Courcelle's theorem \cite{Courcelle1990}, a meta-algorithm for solving problems definable in monadic second-order logic (MSO) on graphs with bounded treewidth in linear time.
%
In particular, we consider an extension of Courcelle's theorem by Arnborg, Lagergren, and Seese, which gives a linear-time algorithm for solving \emph{linear extended MSO extremum problems} on bounded treewidth graphs \cite{ArnborgLagergrenSeese91}. 
%
In \cref{sec:mso-background}, we define MSO logic and give other necessary background before restating \cref{thm:linemsol}, the aforementioned extension of Courcelle's theorem.
%
In \cref{sec:mso-alg}, we show that REIC can be formulated as a linear extended MSO extremum problem and hence solved in $O(n)$ time on rational-weighted graphs of bounded treewidth when budget $r$ is constant. 
%
Notably, both Courcelle's theorem and our DP algorithms are FPL in parameters~$(k,r)$, where $k=\tw(G)$.
%
However, we give three advantages of our tailor-made DP algorithm for REIC over the meta-algorithm.

On the theoretical side, Courcelle's theorem imposes two restrictions on instance structure that our DP algorithms do not require.
%
First, we observe that the MSO logic underlying Courcelle's theorem limits function evaluation to integers.
%
Thus, \cref{thm:linemsol} can only be applied to instances where customers take on rational weights, whereas our DP algorithms allow real-weighted instances.
%
Second, due to its dependence on formula size,  Courcelle's theorem only guarantees an FPT runtime if budget constraint $r$ is constant.
%
Generally, for an MSO formula $\psi$, \cref{thm:linemsol} gives an algorithm with time complexity $O(f(k,|\psi|)\cdot n)$, where automaton size $f$ is a computable function depending on the treewidth $k$ and the formula size $|\psi|$.
%
Although $f(k,|\psi|)=O(1)$ when $k$ and $|\psi|$ are constant, the function $f$ can be exponential\footnote{Indeed, unless $\textup{P}=\textup{NP}$, $f$ cannot be bounded by any elementary function \cite{FrickGrohe04}.} in these parameters.
%
In our case, the MSO formula $\varphi_r$ for REIC-sat relies on the formula $\text{Card}_{=r}$ for verifying the interdiction strategy satisfies the budget constraint. 
%
While $|\text{Card}_{=r}|$ has quadratic dependence on $r$ in our naïve construction, it is clear that any construction for $\text{Card}_{=r}$, and hence for $\varphi_r$, has formula size dependent on~$r$.
%
Thus, Courcelle's theorem does not give an FPT algorithm for REIC for any $r=\omega(1)$;
%
in contrast, our DP algorithms achieve time complexity at worst $O(n^3)$ when treewidth $k$ is bounded.



This dependence of automaton size $f(k,|\varphi_r|)$ on formula size $|\varphi_r|$ also leads to a convincing advantage in practical efficiency for our DP algorithms, due to the large hidden constants hiding in this $O(1)$-term.
%
Putting aside the MSO formula $\text{Card}_{=r}$, our REIC satisfaction formula $\varphi_r$ requires 5 quantifiers to express the disconnection of customers.
%
Based on a lower bound for first-order logic formulas with treewidth 1 conditioned on $\textup{W}[1]\neq \textup{FPT}$ \cite{FrickGrohe04} and an upper bound for MSO formulas with 4 quantifiers \cite[see \cite{KneisLanger09}]{weyer08}, we have the following bounds on the runtime of \cref{thm:linemsol} for our REIC formulation:
\begin{equation*}
2^{2^{2^{2^{\Omega(|\varphi_r|)}}}}\leq O(f(k,|\varphi_r|)\cdot n)\leq 2^{2^{2^{(k+4)^{|\varphi_r|}}}}\ .
\end{equation*}
Therefore, despite having fixed-parameter linear complexity, Courcelle's theorem suffers from extremely large hidden constants in practice.\footnote{For some intuition on this blow-up of automaton size, \cite{KneisLangerRossmanith11} observes that each quantifier alternation requires a power set construction for the automaton; in our case, the formula $\varphi_r$ for REIC-sat involves two quantifier alternations (from $\forall$ to $\exists$ to $\forall$).}
%
As noted by Kneis and Langer, these constants are the barrier to there being a practical implementation of Courcelle's theorem
%%%``the reason why there is de facto no practical implementation of Courcelle’s Theorem available'' 
\cite{KneisLanger09}.    

In summary, while the meta-algorithm of Courcelle's theorem can be applied to REIC on bounded treewidth graphs so long as weights are rational and budget is constant, our DP approach unconditionally offers a direct and computationally efficient algorithm for this problem. We demonstrate our approach's empirical effectiveness in our numerical study of \myAlgorithm in \cref{sec:experimental}, and while we did not implement \ourAlgorithm for bounded treewidth graphs, we expect it be similarly performant due to the shared DP structure and FPL complexity with our algorithm for trees.







==> sections/pseudocode.tex <==
\SetKwProg{Fn}{Function}{}{end}%
\SetKwFunction{FI}{FI}%

\begin{algorithm}[H]
\caption{$r$-Edge Interdiction Covering on Trees}\label{alg:edge-trees}
\DontPrintSemicolon
\Fn{\FI{$T$, $v$, $S$, $w$, $r$}}{
\SetAlgoLined
\SetKwInOut{KwIn}{Input}
\SetKwInOut{KwOut}{Output}

\KwIn{tree $T=(V,E)$ rooted at node $v$, a set of facilities $S$, a customer weight function $w:V\setminus S\rightarrow \mathbb{R}_{\geq 0}$, and an integer budget $r$}
\KwOut{optimal solution values $V$ for REIC on subtree of $T$ rooted at $v$ for budgets $b\leq r$ for all conditions $XY$, predecessor array $P$ and interdiction array $I$ for reconstruction}
\eIf{$v$ is a leaf}{
$P[v,\cdot\ ],I[v,\cdot\ ]\gets \emptyset$

    \For{$b\gets0$ \KwTo $r$}{
\For{$XY\in \{00,01,10,11\}$}{
Calculate $V_{XY}[v,b]$ from base cases
}
}
    }{
$u_1,\ldots,u_k\gets$ children of $v$ in $T$\;
\For{$i\gets1$ \KwTo $k$}{
$V[u_i,\cdot\ ],P[u_i,\cdot\ ], I[u_i,\cdot\ ]\gets $\FI{$T_{u_i}$, $u_i$, $S$, $w$, $r$}\;
}
\For{$b\gets0$ \KwTo $r$}{

\For{$XY\in \{00,01,10,11\}$}{
Calculate $V_{XY}[v,b],P_{XY}[v,b], I_{XY}[v,b]$ from values $V[u_i,\cdot\ ]$ according to recursive DP equations
}
}}

\Return{$V[v,\cdot\ ],P[v,\cdot\ ], I[v,\cdot\ ]$}  
}
\end{algorithm}
